The steady-states of splitter networks

We introduce splitter networks, which abstract the behavior of conveyor belts found in the video game Factorio. Based on this definition, we show how to compute the steady-state of a splitter network. Then, leveraging insights from the players community, we provide multiple designs of splitter networks capable of load-balancing among several conveyor belts, and prove that any load-balancing network on $n$ belts must have $\Omega(n \log n)$ nodes. Incidentally, we establish connections between splitter networks and various concepts including flow algorithms, flows with equality constraints, Markov chains and the Knuth-Yao theorem about sampling over rational distributions using a fair coin.

==> definitions.tex <==
\subsection{Discrete splitter network}

\begin{definition}
  A \emph{discrete splitter network} is a pair $(G, l)$ of a directed
  graph $G$ and a length function $l : E(G) \to \mathbb{N}$, such that
  the vertex set can be partitioned into three sets
  $V(G) = I \disunion S \disunion O$, where:
  \begin{enumerate}[label=(\roman*),noitemsep]
  \item any vertex $i \in I$ is called an \emph{input} and
    satisfies $d^+(i) = 1$, $d^-(i) = 0$,
  \item any vertex $o \in O$ is called an \emph{output} and
    satisfies $d^-(o) = 1$, $d^+(o) = 0$,
  \item any vertex $s \in S$ is called a \emph{splitter} and
    satisfies $d^-(s) = d^+(s) = 2$.
  \end{enumerate}
\end{definition}

Discrete splitter networks modelize conveyor belt networks with
discrete items. The length of an arc represents how many items the
corresponding belt may simultaneously carry. Input and output nodes
represent respectively the entry and exit points of the conveyor
networks, and splitters are devices responsible for balancing the
charges between two conveyor belts. Notice that we allow $G$ to have
loops or parallel arcs.

During usage, many items can be transported at any time by the
conveyor belt network. Each belt has as many slots as its length,
where each slot may contain zero or one item. Nodes cannot hold items,
so the positions of every items are completely determined by which
slots of each belt are occupied. The position of items is not enough
to characterize the state of the network, as each splitter possesses
two bits of internal memory used to try to balance the throughputs
between incident arcs.


\begin{definition}
  A \emph{discrete belt configuration} for a discrete splitter network
  $\displitnetwork$ is a pair
  $(\mathcal{I}, \mathcal{S})$ where 
  \begin{enumerate}[label=(\roman*),noitemsep]
  \item $\mathcal{I}$ is a family $(I_e)_{e \in E(G)}$ with
    $I_e \in \interval{1}{l(e)}$ for any arc $e \in E$. $I_e$ represents
    which slots of belt $e$ contain an item.
  \item $\mathcal{P}$ is a family $(p_s)_{s \in S}$ where
    $p_s \in \delta^-(s) \times \delta^+(s)$. 
  \end{enumerate}
\end{definition}

The dynamic of the conveyor belt networks is given by alternatively
updating along two update methods: belts update and nodes updates.
During a belt update, every item on a belt moves forward to the next
slot (its index decreases), except for those items that are already
accumulating on the most forward slots and which cannot move further.


\begin{definition}
  Given a discrete splitter network $\displitnetwork$ and a discrete
  belt configuration $(\mathcal{I}, \mathcal{P})$, the \emph{outcome
    of a belt update} is a discrete belt configuration
  $(\mathcal{I}', \mathcal{P})$ where
  $$I'_e = \left\{i \in I_e~:~\interval{1}{i} \in I_e\right\} 
         \cup \left\{i~:~ i+1 \in I_e \land \interval{1}{i} \nsubseteq I_e \right\}.$$
\end{definition} 


Nodes updates depend on which input and output nodes are
\emph{active}, and are better described by defining for each node on
which arc it consumes or produces items.

Let $i$ be an input node, with $\delta^+(i) = \{e\}$. If $i$ is active
and $l(e) \notin I_e$, then $i$ produces on $e$. Otherwise $i$ does
not produce on any arc. An input node never consumes.

Let $o$ be an output node, with $\delta^-(o) = \{e\}$. If $o$ is
active and $1 \in I_e$, then $o$ consumes from $e$. Otherwise $o$ does
not consume from any arc. An output node never produces.


Let $s \in S$ be a splitter node, $\{e_1, e_2\} = \delta^-(s)$ and
$\{e_3,e_4\} = \delta^+(s)$ such that $p_s = (e_1,e_3)$. The primary
goal of a splitter node is to maximize its throughput. While
respecting this first constraint, it also tries to balance the
throughputs of incident arcs. To do so, a splitter uses only two bits
of internal memory, to store on which arc it will preferably take the
next item, and on which arc it will preferably put the next item. This
defines a balancing mechanism where the splitter alternates as much as
possible between the two inputs and between the two outputs. The pair
$p_s$ represents the next preferences for a splitter $s$, for instance
$p_s = (e_1,e_3)$ means that the splitter $s$ will rather consumes an item
from $e_1$ and produces an item on $e_3$ during the next update.

The behavior of a splitter $s$ with $p_s = (e_1,e_3)$ is detailed in
Figure~\ref{fig:splitter-array}.


\begin{figure}
  \begin{center}
    \begin{tabular}{cccc|ccc}
      $1 \in I_{e_1}$ & $1 \in I_{e_2}$ & $l(e_3) \in I_{e_3}$ & $l(e_4) \in I_{e_4}$ 
      & $p'_s$ & produces & consumes \\ \hline
      false & false & * & * & $(e_1,e_3)$ & $\emptyset$ & $\emptyset$ \\
      * & * & true & true & $(e_1,e_3)$ & $\emptyset$ & $\emptyset$ \\
      true & true & false & false & $(e_1,e_3)$ & $\{e_1, e_2\}$ & $\{e_3,e_4\}$ \\
      true & * & false & * & $(e_2,e_4)$ & $\{e_1\}$ & $\{e_3\}$ \\
      false & true & false & * & $(e_1,e_4)$ & $\{e_2\}$ & $\{e_3\}$ \\
      true & * & true & false & $(e_2,e_3)$ & $\{e_1\}$ & $\{e_4\}$ \\
      false & true & true & false & $(e_1,e_3)$ & $\{e_2\}$ & $\{e_4\}$ \\
    \end{tabular}
  \end{center}
  \caption{Definitions of which arcs are consumed from or produced to
    by a splitter during an update, and the next preferences of that
    splitter. We assume that $p_s = (e_1,e_3)$. The symbol * stands
    for any value. }
  \label{fig:splitter-array}
\end{figure}

Now that for each node we have defined where is consumes from and
where is produces on, we may define the node update.

\begin{definition}
  Given a discrete splitter network $\displitnetwork$, a discrete belt
  configuration $(\mathcal{I}, \mathcal{S})$ and a set of \emph{active nodes}
  $A \in I \cup O$, the \emph{outcome of a node update} is a discrete
  belt configuration $(\mathcal{I}', \mathcal{S}')$ where
  \begin{enumerate}[label=(\roman*),noitemsep] 
  \item $\mathcal{I}' = (I'_e)_{e \in E}$ where for any $e = uv \in E$,
    $$I'_e = \left\{ 
      \begin{array}{ll}
        I_e \cup \{l(e)\} \setminus \{1\} & \textrm{if $u$ produces on $e$ and $v$ consumes from $e$,}\\
        I_e \cup \{l(e)\} & \textrm{if $u$ produces on $e$,}\\
        I_e \setminus \{1\} & \textrm{if $v$ consumes from $e$,}\\
        I_e & \textrm{otherwise.}
      \end{array}
    \right.
    $$
  \item $\mathcal{S}' = (p'_s)_{s \in S}$ (as described in Figure~\ref{fig:splitter-array}).
  \end{enumerate} 
\end{definition}


Given a set of active nodes $A_t$ for each time step $t$, and an
initial configuration $(\mathcal{I}_0, \mathcal{P}_0)$, one can define
a sequence of configurations over time inductively by applying a belt
update followed by a node update between each time step.


\subsection{Continuous splitter network}

Suppose that the activity of every input or output node is periodic.
As the number of configurations is finite, at some point the
dynamic of the discrete splitter network will also become periodic. It
is then possible to define the average throughput of each arc.
Unfortunately the period may be very long, as it depends on the period
of activity of each node, the length of the arcs and the precise
topology of the directed graph.

In order to study the long-term throughputs of a discrete splitter
network, we introduce a continuous model of a splitter network,
abstracting away the dynamic of the network as well as the length of
each arc. Our hope is that this model will be enough to predict the
throughputs in the discrete splitter network, an hypothesis that will
be tested in Section~\ref{sec:model-comparison}.


\begin{definition}
  A \emph{continuous splitter network} is a directed graph $G$ whose
  vertex set can be partitioned into three sets
  $V(G) = I \disunion S \disunion O$ where
  \begin{enumerate}[label=(\roman*),noitemsep]
  \item any vertex $i \in I$ is called an \emph{input} and
    satisfies $d^+(i) = 1$, $d^-(i) = 0$,
  \item any vertex $o \in O$ is called an \emph{output} and
    satisfies $d^-(o) = 1$, $d^+(o) = 0$,
  \item any vertex $s \in S$ is called a \emph{splitter} and
    satisfies $d^-(s) = d^+(s) = 2$.
  \end{enumerate}
\end{definition}

Given a maximum allowed throughput for each input node and each output
node, our goal is to define the throughput on each arc, as a function
$t : E(G) \to [0,1]$. This requires to establish relationships on the
throughputs of the arcs incident to a splitter node. Recall that we
want the throughputs in the continuous network to be the average
throughputs over a period in the discrete splitter network.

In the discrete settings, the behavior of a belt can be one of two kinds~:
\begin{itemize}[nosep,label=\bull]
\item it may be that all items on the belt move forward at each single
  update (fluid),
\item or there may be some items accumulating at the head of the belt
  (saturated).
\end{itemize}

This affects the behavior of the splitter node who has such an
incoming arc. In particular, it implies that there always is an item
to consume from a saturated belt, hence a splitter node with a
saturated incoming arc will consume at least half of its items from it.
Similarly, a splitter node with a fluid outgoing arc will produce at
least half of its item onto it. If both outgoing arcs are fluid, the
items are evenly distributed, and if both the incoming arcs are
saturated, the items are evenly consumed from both. This imposes rules
on the throughputs of arcs based on the state of the belts, which we
capture with the following definition of an equilibrium.


\begin{definition}
  Let $G = (I \disunion S \disunion O, E)$ be a continuous splitter
  network, and let $c : I \cup O \to [0,1]$ be the maximal capacities
  of each input or output node. An \emph{equilibrium} for $(G,c)$ is a
  pair $(t,F)$ where
  \begin{enumerate}[label=E\arabic*,noitemsep]
  \item \label{eqn:throughput} $t : E \to [0,1]$ is the throughput function,
  \item \label{eqn:fluid-arcs} $F \subseteq E$ is the set of \emph{fluid arcs},
  \item \label{eqn:input-capacity} for each $i \in I$ with $\delta^+(i) = \{e\}$,
    $t(e) \leq c(i)$ and $e \in F \implies t(e) = c(i)$,
  \item \label{eqn:output-capacity} for each $o \in O$ with $\delta^-(o) = \{e\}$,
    $t(e) \leq c(o)$ and $e \notin F \implies t(e) = c(o)$,
  \item \label{eqn:conservation} for each $s \in S$, with
    $\delta^-(s) = \{ e_1, e_2 \}$ and $\delta^+(s) = \{e_3, e_4\}$,
    $t(e_1) + t(e_2) = t(e_3) + t(e_4)$
  \item \label{eqn:incoming-rule} for any $e_1,e_2 \in E$ with
    $\{e_1, e_2\} = \delta^-(s)$ and $e_1 \notin F$,
    $ t(e_1) \geq t(e_2)$
  \item \label{eqn:outgoing-rule} for any $e_1, e_2 \in E$ with
    $\{e_1, e_2\} = \delta^+(s)$ and $e_1 \in F$, $t(e_1) \geq t(e_2)$
  \item \label{eqn:maximization} for any $uv \in E \setminus F$ and
    $vw \in F$, $t(uv) = 1$ or $t(vw) = 1$.
  \end{enumerate}
\end{definition}



In the continuous setting, we will use the word \emph{flow} to
informally describe the material transported by the network, that is
the continuous analog of the items. Rules~\ref{eqn:input-capacity}
and~\ref{eqn:output-capacity} say that the throughputs are limited at
each input and each ouput, and moreover, an input pushes as much flow
as possible up to its capacity or until the outgoing arc is saturated.
Similarly an output absorbs as much flow as possible, up to its
capacity, which means that the incoming arc cannot be saturated unless
its throughput equals the output capacity.

Rule~\ref{eqn:conservation} imposes the conservation of flow (items
cannot be stored in splitters). Rules~\ref{eqn:incoming-rule}
and~\ref{eqn:outgoing-rule} enforce the balancing constraints: a
splitter consumes no less flow from a saturated arc than from another
incoming arc, and produces no less flow in a fluid outgoing arc than
in another outgoing arc. In particular, if both incoming arcs are
saturated, or if both outgoing arcs are fluid, they must have equal
throughput. 

\begin{definition}
  Given a continuous splitter network $\splitnetwork$ and a set
  $F \subseteq E$ of fluid arcs, we say that two arcs $e, e' \in E$
  are 
  \begin{itemize}[label=\bull,nosep]
  \item \emph{in-coupled} if $e, e' \notin F$ and there is a splitter
    vertex $v \in S$ with $\delta^-(v) = \{e, e'\}$,
  \item \emph{out-coupled} if $e, e' \in F$ and there is a splitter
    vertex $v \in S$ with $\delta^+(v) = \{e, e'\}$,
  \item \emph{coupled} if they are in-coupled or out-coupled.
  \end{itemize}
\end{definition}


Finally rule~\ref{eqn:maximization} imposes the
maximisation of the throughput by each splitter: if an arc entering a
splitter is saturated, the splitter must use as much flow as possible
from that arc. Rule~\ref{eqn:maximization} can be rewritten in a form
that emphasizes the goal of maximizing the splitter throughput:



\begin{lemma}
  Let $\splitnetwork$ be a continuous splitter network,
  $F \subseteq E$ and $t : E \to [0,1]$. Suppose that for any $s \in S$,
  $\sum_{e \in \delta^-(v)} t(e) = \sum_{e \in \delta^+(v)} t(e).$
  Then the two following propositions are equivalent:
  \begin{enumerate}[label=(\arabic*),noitemsep]
  \item\label{item:max1} for any arcs $uv \in F$ and $vw \notin F$,
    $t(uv) = 1$ or $t(vw) = 1$.
  \item\label{item:max2} for any vertex $s \in S$ with
    $\delta^-(s) = \{e_1,e_2\}$ and $\delta^+(e) = \{e_3,e_4\}$,
    $$t(e_1) + t(e_2) = \min \{ \trout_{e_1} + \trout_{e_2}, \trin_{e_3} + \trin_{e_4}\}.$$
  \end{enumerate}
  where for any arc $e$, 
  \begin{equation}
      \trout_e = 
      \left\{ 
        \begin{array}{ll}
          1 & \textrm{if $e \notin F$},\\
          t(e) & \textrm{otherwise}
        \end{array} 
      \right. 
      \qquad\textrm{and}\qquad
      \trin_e = 
      \left\{ 
        \begin{array}{ll}
          1 & \textrm{if $e \in F$},\\
          t(e) & \textrm{otherwise}
        \end{array} 
      \right. 
      \label{eqn:arc-capacities}
  \end{equation} 
\end{lemma}


\begin{proof}
  \ref{item:max1} implies~\ref{item:max2}: If $e_1, e_2 \in F$, then
  $$\trout_{e_1} + \trout_{e_2} = t(e_1) + t(e_2) = t(e_3) + t(e_4) \leq \trin_{e_3} + \trin_{e_4}.$$
  Suppose now that $e_1 \notin F$ and $t(e_1) < 1$. Then for
  $e \in \delta^+(s)$, we have $e \notin F$ or $t(e) = 1$
  by~\ref{item:max1}, thus $\trin_{e} = t(e)$. From this, we get
  $$\trin_{e_3} + \trin_{e_4} = t(e_3) + t(e_4) = t(e_1) + t(e_2) \leq \trout_{e_1} + \trout_{e_2}.$$

  \ref{item:max2} implies~\ref{item:max1}: Let $uv \notin F$ and
    $vw \in F$ with $t(uv) < 1$. Let $u'v$ and $vw'$ the other two
    arcs incident to $v$. Then
    $$\min \{ 1 + \trout_{vw}, \trin_{vw} + \trin_{vw'} \} = t(uv) + t(u'v) < 1 + \trout_{vw'}.$$
    Thus $t(vw) + t(vw') = \trin_{vw} + \trin_{vw'}$ which implies
    that $t(vw) = \trin_{vw} = 1$ because $vw \in F$.
\end{proof}



% as well as the local maximization of
% the throughput. Indeed for a splitter $s$, $T_s$ is the maximum
% throughput realizable by $s$~: it cannot process more than what is
% available in its incoming arcs or what can be absorbed by its outgoing
% arcs. Notice that if an arc is saturated, the splitter can take
% arbitrarily many items (to the limit of one unit per time step). This
% translates into a maximal available throughput of 1 for each saturated
% incoming arc. Similarly, a fluid outgoing arc has an available
% throughput of 1. This is captured by the definition of $\trin_e$ and
% $\trout_e$.


For convenience, when defining or representing discrete or continuous
splitter networks, we will allow splitters with in-degree one or
out-degree one. This is justified by the fact that if a splitter $s$
has in-degree one, we can add an dummy input node $i$ with capacity
$c(i) = 0$ with an arc from $i$ to $s$ that will be always fluid.
Similarly if $s$ has out-degree one, we can add a dummy output node
$o$ with capacity $c(o) = 0$ and an arc from $s$ to $o$ that will
always be saturated. The throughput on those arcs is forced to be $0$,
and it does not create any more constraint on the non-dummy arcs as
rules~\ref{eqn:incoming-rule} and~\ref{eqn:outgoing-rule} are clearly
true for those arcs.

Also for convenience, for any input $i \in I$ with outgoing arc $e$,
we note $t(i) \eqdef t(e)$, and similarly for any output $o \in O$
with incoming arc $e$, $t(o) \eqdef t(e)$. We also extend the capacity to arcs by setting: 
$$ c(e) := \left\{\begin{array}{ll}
c(i) &\quad \textrm{ if $e$ leaves input $i$,}\\
c(o) &\quad \textrm{ if $e$ enters output $o$,}\\
1 &\quad \textrm{ otherwise.}
\end{array}\right.$$


\subsection{Discrepancies between the two definitions, simulation
  results.}\label{sec:model-comparison}

Examples show that the throughputs obtained from the continuous model
is not always achieved by the discrete model. Actually the throughputs
in the discrete model depends on the length of the arcs as well as the
initial configuration, which are abstracted away by the continuous model.

From the few examples tested, it seems that the throughputs predicted
by the continuous model are realizable in the discrete model as long
as we carefully choose the length of the arcs and the initial
configuration.

One reason for the discrepancy between the discrete and continuous
model is that the discrete model do not always pick an item from a
saturated incoming arc at each time step, for instance when the
outgoing arcs only accept one item. Indeed, because the splitter takes
at least half the items from the saturated incoming arcs, its
preference is more often to consume an item from the other incoming
arc, while the continuous model rule~\ref{eqn:incoming-rule} suggests
a preference for the saturated incoming arc.



% Can we guarantee that the discrete throughput is at least half the continuous throughput ?

% Prove that discrete throughput <= continuous throughput. 
% By taking the average throughput on each arc during the periodic
% cycle and showing that this is dominated by a continuous solution?


